FixEval: Execution-based Evaluation of Program Fixes for Programming Problems

The complexity of modern software has led to a drastic increase in the time and cost associated with detecting and rectifying software bugs. In response, researchers have explored various methods to automatically generate fixes for buggy code. However, due to the large combinatorial space of possible fixes for any given bug, few tools and datasets are available to evaluate model-generated fixes effectively. To address this issue, we introduce FixEval, a benchmark comprising of buggy code submissions to competitive programming problems and their corresponding fixes. FixEval offers an extensive collection of unit tests to evaluate the correctness of model-generated program fixes and assess further information regarding time, memory constraints, and acceptance based on a verdict. We consider two Transformer language models pretrained on programming languages as our baseline and compare them using match-based and execution-based evaluation metrics. Our experiments show that match-based metrics do not reflect model-generated program fixes accurately. At the same time, execution-based methods evaluate programs through all cases and scenarios designed explicitly for that solution. Therefore, we believe FixEval provides a step towards real-world automatic bug fixing and model-generated code evaluation. The dataset and models are open-sourced at https://github.com/mahimanzum/FixEval.

==> figure/java_generations.tex <==

%\toufique{made some space between the two image}

\begin{table}[H]
\vspace{2mm}
\caption{Some Java examples which were also successfully generated by our model when we pass the buggy code to it. The errors are marked with red}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Model learned to copy entire line out of scope}  \vspace{1mm}\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:} \\ 

~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} D = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} N = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a;} \\ 
~~~~~~~~~~\texttt{a = (\textcolor{blue}{int}) Math.pow(\textcolor{blue}{100}, D )*N;} \\ 
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (N == 100)\{ } \\ 
~~~~~~~~~~~~~~\texttt{a = (\textcolor{blue}{int}) Math.pow(\textcolor{blue}{100}, D)*(N+1);\} } \\ 
~~~~~~~~~~~~~~\texttt{\textcolor{red}{\st{System.out.println(a);}}} \\ 
~~~~~~~~~~\texttt{\} } \\ 
~~\texttt{\} } \\ 
~ \\
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} D = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} N = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a;} \\ 
~~~~~~~~~~\texttt{a = (\textcolor{blue}{int}) Math.pow(\textcolor{blue}{100}, D )*N;} \\ 
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (N == 100)\{ } \\ 
~~~~~~~~~~~~~~\texttt{a = (\textcolor{blue}{int}) Math.pow(\textcolor{blue}{100}, D)*(N+1);\} } \\ 
~~~~~~~~~~\texttt{\} } \\ 
~~~~~~~~~~\texttt{System.out.println(a);} \\ 
~~\texttt{\} } \\ 
~ \\
\end{tabular} \\ \hline




\hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Model learned change logic from or to and}  \vspace{1mm}\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} b = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} ( a <= \textcolor{blue}{8} \textcolor{red}{\st{||}} b <= \textcolor{blue}{8} ) \{}\\
~~~~~~~~~~~~~~\texttt{System.out.println(\textcolor{orange}{"Yay!"});}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~~~~~\texttt{\textcolor{magenta}{else} \{}\\
~~~~~~~~~~~~~~\texttt{System.out.println(\textcolor{orange}{":(")};}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~ \\
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} b = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} ( a <= \textcolor{blue}{8} \&\& b <= \textcolor{blue}{8} ) \{}\\
~~~~~~~~~~~~~~\texttt{System.out.println(\textcolor{orange}{"Yay!"});}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~~~~~\texttt{\textcolor{magenta}{else} \{}\\
~~~~~~~~~~~~~~\texttt{System.out.println(\textcolor{orange}{":(" )};}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~ \\
\end{tabular} \\ \hline





\vspace{-4mm}\\ \hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Model Learned to change return statement to a print statement} 
\vspace{1mm}
\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:}  \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} a2 = a * a;}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} a3 = a2 * a;}\\
~~~~~~~~~~\texttt{\textcolor{blue}{ \textcolor{red}{\st{return}}} a + a2 + a3;}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~ \\
\end{tabular}} & 
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc.nextInt();}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} a2 = a * a;}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} a3 = a2 * a;}\\
~~~~~~~~~~\texttt{System.out.println( a + a2 + a3 );}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~ \\
\end{tabular}
\\ \hline
\vspace{-2mm}\\




\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Model Learned to change syntax and compilation error} 
\vspace{1mm}
\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:}  \\ 
\texttt{ \textcolor{magenta}{import} java.util.*} \\ 
~~\texttt{\textcolor{magenta}{ public class } \textcolor{cyan}{Main} \{ } \\ 
~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String} [] args)\{} \\ 
~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~\texttt{\textcolor{blue}{int} A = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} B = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} T = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} S = \textcolor{red}{\st{T/A} }System.out.println(s*\textcolor{red}{\st{b}});} \\
~~~~\texttt{\}} \\  
~~\texttt{\}}  
\end{tabular}} & 
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
\texttt{ \textcolor{magenta}{import} java.util.*} \\ 
~~\texttt{\textcolor{magenta}{ public class } \textcolor{cyan}{Main} \{ } \\ 
~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String} [] args)\{} \\ 
~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~\texttt{\textcolor{blue}{int} A = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} B = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} T = sc.nextInt();} \\
~~~~~~~\texttt{\textcolor{blue}{int} S = T/A;}\\
~~~~~~~\texttt{System.out.println(s*B);} \\
~~~~\texttt{\}} \\  
~~\texttt{\}}  
\end{tabular}
\\ \hline
\vspace{-2mm}\\



\end{tabular}%
}


\label{tab:examples_java}
\vspace{-6mm}
\end{table}


==> figure/java_generations_mint.tex <==
\begin{figure*}[t]
\centering

\vspace{5pt}

\begin{tabular}{p{13.5cm}}
\toprule
Model learned to copy entire line out of scope\\
\bottomrule
\end{tabular}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program (Wrong Answer)}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=11
        \color{red!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int D = sc.nextInt();
        int N = sc.nextInt();
        int a;
        a = (int) Math.pow(100, D )*N;
        if (N == 100){
            a = (int) Math.pow(100, D)*(N+1);
            System.out.println(a);
        }
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=12
            \color{green!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int D = sc.nextInt();
        int N = sc.nextInt();
        int a;
        a = (int) Math.pow(100, D )*N;
        if (N == 100){
            a = (int) Math.pow(100, D)*(N+1);
        }
        System.out.println(a);
    }
}
\end{lstlisting}



\end{tabular}
\end{adjustbox}
\end{tabular}



\centering

\vspace{5pt}

\begin{tabular}{p{13.5cm}}
\toprule
Model learned change logic from "or" to "and" \\
\bottomrule
\end{tabular}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program (Wrong Answer)}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=7
        \color{red!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int a = sc.nextInt();
        int b = sc.nextInt();
        if ( a <= 8 || b <= 8 ) {
            System.out.println("Yay!");
        }
        else {
            System.out.println(":(");
        }
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=7
            \color{green!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int a = sc.nextInt();
        int b = sc.nextInt();
        if ( a <= 8 && b <= 8 ) {
            System.out.println("Yay!");
        }
        else {
            System.out.println(":(");
        }
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}



\centering
\vspace{5pt}
\begin{tabular}{p{13.5cm}}
\toprule
Model Learned to change return statement to a print statement \\
\bottomrule
\end{tabular}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program (Compilation Error)}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=8
        \color{red!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int a = sc.nextInt();
        int a2 = a * a;
        int a3 = a2 * a;
        return a + a2 + a3;
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=8
            \color{green!10}
    \fi
    }
]
import java.util.*;
public class Main {
    public static void main(String[] args){
        Scanner sc = new Scanner(System.in);
        int a = sc.nextInt();
        int a2 = a * a;
        int a3 = a2 * a;
        System.out.println( a + a2 + a3 );
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}




\centering
\vspace{5pt}
\begin{tabular}{p{13.5cm}}
\toprule
Model Learned to change syntax and compilation error \\
\bottomrule
\end{tabular}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program (Compilation Error)}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=8
        \color{red!10}
    \fi
    }
]
import java.util.*
public class Main {
    public static void main(String [] args){
        Scanner sc = new Scanner(System.in);
        int A = sc.nextInt();
        int B = sc.nextInt();
        int T = sc.nextInt();
        int S = T/A System.out.println(s*b);
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=8
            \color{green!10}
    \fi
    \ifnum\value{lstnumber}=9
            \color{green!10}
    \fi
    }
]
import java.util.*
public class Main {
    public static void main(String [] args){
        Scanner sc = new Scanner(System.in);
        int A = sc.nextInt();
        int B = sc.nextInt();
        int T = sc.nextInt();
        int S = T/A;
        System.out.println(s*B);
    }
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}

\caption{
Examples of successful fixes of buggy programs in Java. Buggy and fixed statements are marked in red and green, respectively.
}
\label{fig:examples_java}
\end{figure*}


==> figure/python_generations.tex <==

%\toufique{made some space between the two image}

\begin{table}[H]
\vspace{2mm}
\caption{Some Python examples which were also successfully generated by our model when we pass the buggy code to it. The errors are marked with red}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Model learned to cast the output}  \vspace{1mm}\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:} \\ 
~~\texttt{n =  \textcolor{blue}{int}(\textcolor{blue}{input}()) } \\ 
~~\texttt{n =  \textcolor{blue}{print}( \textcolor{red}{\st{int}} (n-1+1)*(n-1)/2)} \\ 
~ \\
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{n =  \textcolor{blue}{int}(\textcolor{blue}{input}()) } \\ 
~~\texttt{n =  \textcolor{blue}{print}(\textcolor{blue}{int}((n-1+1)*(n-1)/2))} \\ 
~ \\
\end{tabular} \\ \hline




\hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{Model learned add sort function correctly}  \vspace{1mm}\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:} \\ 
~~\texttt{n =  \textcolor{blue}{int}(\textcolor{blue}{input}()) } \\ 
~~\texttt{a =  \textcolor{blue}{list}(\textcolor{blue}{map}(\textcolor{blue}{int},\textcolor{blue}{input}\char`\\} \\
~~~~~~~~\texttt{().split())).\textcolor{red}{\st{sort()}}} \\
~~\texttt{\textcolor{blue}{print}(a[-1]-a[0])} \\
~ \\
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{n =  \textcolor{blue}{int}(\textcolor{blue}{input}()) } \\ 
~~\texttt{a =  \textcolor{blue}{list}(\textcolor{blue}{map}(\textcolor{blue}{int},\textcolor{blue}{input}.split()))} \\
~~\texttt{a.sort()} \\
~~\texttt{\textcolor{blue}{print}(a[-1]-a[0])} \\
~ \\
\end{tabular} \\ \hline





\vspace{-4mm}\\ \hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Model Learned to change the comparison sign} 
\vspace{1mm}
\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:}  \\ 
~~\texttt{N, K = \textcolor{blue}{map}(\textcolor{blue}{int}, \textcolor{blue}{input}().split()) } \\ 
~~\texttt{h = \textcolor{blue}{input}().split() } \\ 
~~\texttt{c = 0 } \\
~~\texttt{\textcolor{magenta}{for} i \textcolor{magenta}{in} \textcolor{blue}{range}(N) } \\
~~~~\texttt{ \textcolor{magenta}{if} \textcolor{blue}{int}(h[i]) \textcolor{red}{\st{>}} k :  } \\ 
~~~~~~\texttt{c += 1} \\ 
~~\texttt{\textcolor{blue}{print}(c)} 
~ \\
\end{tabular}} & 
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{N, K = \textcolor{blue}{map}(\textcolor{blue}{int}, \textcolor{blue}{input}().split()) } \\ 
~~\texttt{h = \textcolor{blue}{input}().split() } \\ 
~~\texttt{c = 0 } \\
~~\texttt{\textcolor{magenta}{for} i \textcolor{magenta}{in} \textcolor{blue}{range}(N) } \\
~~~~\texttt{ \textcolor{magenta}{if} \textcolor{blue}{int}(h[i]) \textcolor{teal}{>=} k :  } \\ 
~~~~~~\texttt{c += 1} \\ 
~~\texttt{\textcolor{blue}{print}(c)}\\
~ \\
\end{tabular}
\\ \hline
\vspace{-2mm}\\


\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{Model Learned to change loop range for corrcetion} 
\vspace{1mm}
\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:}  \\ 
~~\texttt{\textcolor{magenta}{from} collections \textcolor{magenta}{import} defaultdict } \\ 
~~\texttt{N = \textcolor{blue}{int}(\textcolor{blue}{input}())} \\ 
~~\texttt{d = defaultdict(\textcolor{blue}{int})} \\
~~\texttt{\textcolor{magenta}{for} n \textcolor{magenta}{in} \textcolor{blue}{range}(\textcolor{red}{\st{N}}):} \\
~~~~~~\texttt{n = \textcolor{blue}{str}(n)} \\
~~~~~~\texttt{a = n[0]} \\
~~~~~~\texttt{b = n[- 1]} \\
~~~~~~\texttt{d[(a,b)]+=1} \\
~~\texttt{s = 0} \\
~~\texttt{\textcolor{magenta}{for} i \textcolor{magenta}{in} \textcolor{blue}{range}(1,10):} \\
~~~~~~\texttt{\textcolor{magenta}{for} j \textcolor{magenta}{in} \textcolor{blue}{range}(10):} \\
~~~~~~~~~~\texttt{s += d[(\textcolor{blue}{str}(j), \textcolor{blue}{str}(i))]* \char`\\} \\ 
~~\texttt{d[(\textcolor{blue}{str}(i), \textcolor{blue}{str}(j))]} \\
~~\texttt{\textcolor{blue}{print}(s)} \\
~ \\
\end{tabular}} & 
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{from} collections \textcolor{magenta}{import} defaultdict } \\ 
~~\texttt{N = \textcolor{blue}{int}(\textcolor{blue}{input}())} \\ 
~~\texttt{d = defaultdict(\textcolor{blue}{int})} \\
~~\texttt{\textcolor{magenta}{for} n \textcolor{magenta}{in} \textcolor{blue}{range}(\textcolor{blue}{N+1}):} \\
~~~~~~\texttt{n = \textcolor{blue}{str}(n)} \\
~~~~~~\texttt{a = n[0]} \\
~~~~~~\texttt{b = n[- 1]} \\
~~~~~~\texttt{d[(a,b)]+=1} \\
~~\texttt{s = 0} \\
~~\texttt{\textcolor{magenta}{for} i \textcolor{magenta}{in} \textcolor{blue}{range}(1,10):} \\
~~~~~~\texttt{\textcolor{magenta}{for} j \textcolor{magenta}{in} \textcolor{blue}{range}(10):} \\
~~~~~~~~~~\texttt{s += d[(\textcolor{blue}{str}(j), \textcolor{blue}{str}(i))]* \char`\\} \\ 
~~\texttt{d[(\textcolor{blue}{str}(i), \textcolor{blue}{str}(j))]} \\
~~\texttt{\textcolor{blue}{print}(s)} \\
~ \\
\end{tabular}
\\ \hline
\vspace{-2mm}\\



\end{tabular}%
}
\label{tab:example_2_python}
\vspace{-6mm}
\end{table}


==> figure/python_generations_mint.tex <==
\begin{figure*}[t]
\centering


\begin{tabular}{p{13.5cm}}
\toprule
Model learned to cast the output \\
\bottomrule
\end{tabular}


\vspace{5pt}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program in Python}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=2
        \color{red!10}
    \fi
    }
]
n = int(input())
n = print(int(n-1+1)*(n-1)/2)
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program in Python}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=2
            \color{green!10}
    \fi
    }
]
n = int(input())
n = print(int((n-1+1)*(n-1)/2))
\end{lstlisting}



\end{tabular}
\end{adjustbox}
\end{tabular}
\vspace{6mm}

\begin{tabular}{p{13.5cm}}
\toprule
Model learned add sort function correctly \\
\bottomrule
\end{tabular}


\centering

\vspace{5pt}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program in Python}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=3
        \color{red!10}
    \fi
    }
]
n = int(input())
a = list(map(int,input().split())).sort()
print(a[-1]-a[0])

\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program in Python}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=3
            \color{green!10}
    \fi
    }
]
n = int(input())
a = list(map(int,input.split()))
a.sort()
print(a[-1]-a[0])

\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}





\vspace{6mm}

\begin{tabular}{p{13.5cm}}
\toprule
Model Learned to change the comparison sign \\
\bottomrule
\end{tabular}


\centering

\vspace{5pt}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program in Python}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=5
        \color{red!10}
    \fi
    }
]
N, K = map(int, input().split())
h = input().split()
c = 0
for i in range(N):
    if int(h[i]) > k:
        c += 1
print(c)
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program in Python}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=5
            \color{green!10}
    \fi
    }
]
N, K = map(int, input().split())
h = input().split()
c = 0
for i in range(N):
    if int(h[i]) > k:
        c += 1
print(c)
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}



\vspace{6mm}

\begin{tabular}{p{13.5cm}}
\toprule
Model Learned to change loop range for corrcetion\\
\bottomrule
\end{tabular}


\centering

\vspace{5pt}
\begin{tabular}{l}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Buggy Program in Python}
\end{center}
\begin{tabular}{l}


\lstset{escapechar=~,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=4
        \color{red!10}
    \fi
    }
]
from collections import defaultdict
N = int(input())
d = defaultdict(int)
for n in range(N):
    n = str(n)
    a = n[0]
    b = n[- 1]
    d[(a,b)] += 1
s = 0
for i in range(1, 10):
    for j in range(10):
        s += d[(str(j), str(i))] * d[(str(i), str(j))]
print(s)
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\hspace{8pt}
% \vspace{10pt}
\begin{adjustbox}{valign=t,minipage=0.47\textwidth}
\begin{center}
    \underline{Fixed Program in Python}
\end{center} 
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}[ 
    linebackgroundcolor={%
    \ifnum\value{lstnumber}=4
            \color{green!10}
    \fi
    }
]
from collections import defaultdict
N = int(input())
d = defaultdict(int)
for n in range(N+1):
    n = str(n)
    a = n[0]
    b = n[- 1]
    d[(a,b)]+=1
s = 0
for i in range(1,10):
    for j in range(10):
        s += d[(str(j), str(i))] * d[(str(i), str(j))]
print(s)
\end{lstlisting}
\end{tabular}
\end{adjustbox}
\end{tabular}

\caption{
Examples of successful fixes of buggy programs in Python. Buggy and fixed statements are marked in red and green, respectively.
}
\label{fig:example_2_python}
\end{figure*}


==> figure/solved_with_verdict.tex <==
%\toufique{made some space between the two image}

\begin{table}[H]
\caption{Java examples from the sampled \textsc{FixEval} test set that were only successfully solved with the verdict information as conditional model input.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\hline
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}} \textbf{From the verdict information, the model learned to change the type to be consistent with \texttt{\textcolor{blue}{long}}\vspace{1mm}}  \end{tabular}} \\ \hline
\addlinespace[1ex]
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code: } \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{import} java.lang.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{\st{int}} a = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{\st{int}} b = sc.nextInt();} \\
~~~~~~~~~~\texttt{\textcolor{blue}{long} ans = a*b/gcd(a, b)} \\
~~~~~~~~~~\texttt{System.out.println(ans);} \\
~~~~~~~~~~\texttt{sc.close()} \\
~~~~~~\texttt{\} } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{long} \textcolor{cyan}{gcd}(long m,long n)\{ } \\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (m < n) \textcolor{magenta}{return} gcd(n, m)} \\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (n==0) \textcolor{magenta}{return} m} \\
~~~~~~~~~~\texttt{\textcolor{magenta}{return} gcd(n, m\%n)} \\

~~~~~~~~\texttt{\} } \\ 
~~\texttt{\} } \\ 
~~\texttt{\textbf{\textcolor{orange}{Verdict: Wrong Answer}}} \\ 
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{import} java.lang.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{long} a = sc.nextInt();} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{long} b = sc.nextInt();} \\
~~~~~~~~~~\texttt{\textcolor{blue}{long} ans = a*b/gcd(a, b)} \\
~~~~~~~~~~\texttt{System.out.println(ans);} \\
~~~~~~~~~~\texttt{sc.close()} \\
~~~~~~\texttt{\} } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{long} \textcolor{cyan}{gcd}(long m,long n)\{ } \\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (m < n) \textcolor{magenta}{return} gcd(n, m)} \\
~~~~~~~~~~\texttt{\textcolor{magenta}{if} (n==0) \textcolor{magenta}{return} m} \\
~~~~~~~~~~\texttt{\textcolor{magenta}{return} gcd(n, m\%n)} \\

~~~~~~~~\texttt{\} } \\ 
~~\texttt{\} } \\ 
~ \\
\end{tabular} \\
\hline
\addlinespace[1ex]
\multicolumn{2}{l}{\begin{tabular}[c]{@{}l@{}}\textbf{From the verdict information, the model learned to change variable names that exist in the code}  \vspace{1mm}\end{tabular}} \\ \hline
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Buggy Input Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc . nextInt ( ) ;}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} b = sc . nextInt ( ) ;}\\
~~~~~~~~~~\texttt{if((\st{A} - \st{B}) \% 2  == 0 ) \{ }\\
~~~~~~~~~~~~~~\texttt{System.out.println(( \st{A} + \st{B} )/2)}\\
~~~~~~~~~~\texttt{\}} \\
~~~~~~~~~~\texttt{else \{ }\\
~~~~~~~~~~~~~~\texttt{System.out.println("\textcolor{red}{IMPOSSIBLE}")}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~~\texttt{\textbf{\textcolor{orange}{Verdict: Compilation Error}}} \\ 
\end{tabular}} &
\begin{tabular}[c]{@{}l@{}}
\addlinespace[1ex]
\textbf{Model generated Fixed Code:} \\ 
~~\texttt{\textcolor{magenta}{import} java.util.*;} \\ 
~~\texttt{\textcolor{magenta}{public class} \textcolor{cyan}{Main}\{ } \\ 
~~~~~~\texttt{\textcolor{magenta}{public static} \textcolor{blue}{void} main(\textcolor{blue}{String}[] args)\{ } \\ 
~~~~~~~~~~\texttt{Scanner sc = \textcolor{magenta}{new} Scanner(System.in);} \\ 
~~~~~~~~~~\texttt{\textcolor{blue}{int} a = sc . nextInt ( ) ;}\\
~~~~~~~~~~\texttt{\textcolor{blue}{int} b = sc . nextInt ( ) ;}\\
~~~~~~~~~~\texttt{if((a-b) \% 2  == 0 ) \{ }\\
~~~~~~~~~~~~~~\texttt{System.out.println((a+b)/2)}\\
~~~~~~~~~~\texttt{\}} \\
~~~~~~~~~~\texttt{else \{ }\\
~~~~~~~~~~~~~~\texttt{System.out.println("\textcolor{red}{IMPOSSIBLE}")}\\
~~~~~~~~~~\texttt{\}}\\
~~~~~~\texttt{\}}\\
~~\texttt{\}}\\
~ \\
\end{tabular} \\ \hline

\end{tabular}%
}


\label{tab:solved_with_verdict}
\vspace{-6mm}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/limitations.tex <==
\section{Limitations}

% \textcolor{red}{Move to appendix?} 
There are a few limitations of the dataset presented in this work. In our experiments, we manually analyze the mistakes made by models with and without access to verdict information. We find that common model mistakes include additions of code segments that are unnecessary to fix a given bug. We believe this is due to insufficient information about the bug and the problem. Another limitation of this work is that, while the code bug fix pair dataset can be extended for other programming languages, code, and test suite expansion for more problems is solely dependent upon AtCoder availability. 
Also, the execution-based evaluation metric calculation requires a substantial amount of time to evaluate a single program. To reduce computation complexity, we select two data points randomly per problem from the test dataset. Nevertheless, parallelism and high-performance computing can be utilized towards making execution-based evaluation faster and more efficient for large-scale data.
In terms of research insights, our dataset incorporates Java and Python bugs, and may not generalize to other programming languages. Further research is necessary to evaluate the impact of FixEval for analyzing deep learning models for additional languages. Additionally, competitive programs submitted online may not accurately reflect real-world software bugs from professional developers. More work is necessary to develop benchmarks that simulate authentic software programs to evaluate deep learning models for automated program repair. %\il{In this work, we introduce \textsc{\textbf{FixEval}} as a useful context-aware dataset for evaluating models for bug fixing on programs with varying sizes and difficulties that incorporate space and time constraints.}\il{revise this and contribution \#1 , see the email, possible parsing variants with a different meaning. Does not seem to connect well with the last limitation. Should we skip this part? Or revise to better connect.}

%\todo{In general, need to organize this as: Limitation -> how we mitigate it/why it is necessary}


==> table/4_execution_based_results.tex <==

\begin{table}[t!]
\centering
\begin{subtable}
\resizebox{\linewidth}{!} {%
\def\arraystretch{1.0}%
\begin{tabular}{l c cccc  cccc}
    \toprule
    \multicolumn{2}{c}{} & \multicolumn{4}{c}{pass@$k$} & \multicolumn{4}{c}{top-$k$ TCA} \\
    \cmidrule{3-10}
    Language & Verdict & $ k=1 $ & $ k=3$ & $k=5 $& $k=10$ & $k=1$ & $k=3$ & $k=5$ & $k=10$  \\
    \midrule
    Java & \xmark & 8.65 & 15.62 & 19.63 & 24.44 & 41.00 & 34.00 & 32.70& 29.60\\ 
    Java & \checkmark & \textbf{10.94} & \textbf{18.77} & \textbf{22.66} & \textbf{27.96}& \textbf{44.99} & \textbf{38.80} & \textbf{35.87} & \textbf{32.90} \\ 
    \midrule
    Python &\xmark & 6.86 & 13.07 & 16.27 & 20.51 & \textbf{50.20} & \textbf{41.20} & \textbf{38.50} & \textbf{35.20} \\ 
    Python & \checkmark & \textbf{7.32} & \textbf{13.94} & \textbf{17.47} & \textbf{22.63} & 48.75 & 41.16 & 38.37 & 34.88 \\ 
    \bottomrule
\end{tabular}
}
\caption{Execution-based Results for CodeT5.}
\label{tab:execution_based_results_1}
\end{subtable}

\bigskip
\begin{subtable}
\centering
\begin{tabular}{c c c}
    \toprule
    Language & pass$@1$ & top-$1$ TCA \\
    \midrule
    Java & 0.0 & 37.95 \\ 
    Python & 0.0 & 41.55 \\ 
    \bottomrule
\end{tabular}
\caption{Execution-based Results for Naive Copy.}
\label{tab:execution_based_results_2}
\end{subtable}
\caption{Execution-based evaluation metrics on the sampled evaluation \fixeval.}
\label{tab:execution_based_results}
\end{table}



==> table/bifi_results.tex <==
\begin{wraptable}{R}{50mm}
\begin{tabular}{ cccc } 
 \hline
 \textbf{Category} & \textbf{Error Removal(\%)} \\ \hline
 Wrong answer  & 3.1  \\
 Runtime error & 5.5\\ 
 Time limit exceeded  & 1.8  \\
 Overall  & 3.4 \\
 \hline
\end{tabular}
\captionof{table}{BIFI model accuracy on \fixeval Python test set. \il{which accuracy is this one? TCA?[Their own metric which is Error Removal]}}
\label{tab:Bifi_results}
\end{wraptable}
